Aggregator Reuse and Extension for Richer Web Archive Interaction

Memento aggregators enable users to query multiple web archives for captures of a URI in time through a single HTTP endpoint. While this one-to-many access point is useful for researchers and end-users, aggregators are in a position to provide additional functionality to end-users beyond black box style aggregation. This paper identifies the state-of-the-art of Memento aggregation, abstracts its processes, highlights shortcomings, and offers systematic enhancements.

==> Makefile <==
SHELL=/bin/bash
MAIN=cyclic
LATEX=pdflatex
BIBTEX=bibtex
DTM=$(shell date +%Y%m%d-%H%M%S)

# If the first argument is "run"...
ifeq (chapter,$(firstword $(MAKECMDGOALS)))
  # use the rest as arguments for "chapter"
  CHAPTER_ARGS := $(wordlist 2,$(words $(MAKECMDGOALS)),$(MAKECMDGOALS))
  # ...and turn them into do-nothing targets
  $(eval $(CHAPTER_ARGS):;@:)
endif

all: clean build clear

chapter:
	@echo $(CHAPTER_ARGS)
	CHAPSTR='\def\ischapter{'$(CHAPTER_ARGS)'}'
	$(LATEX) $(CHAPSTR) $(MAIN).tex
	$(BIBTEX) $(CHAPSTR) $(MAIN).tex
	$(LATEX) $(CHAPSTR) $(MAIN).tex
	$(LATEX) $(CHAPSTR) $(MAIN).tex

build:
	$(LATEX) $(MAIN).tex
	$(BIBTEX) $(MAIN)
	$(LATEX) $(MAIN).tex
	$(LATEX) $(MAIN).tex
	@cp $(MAIN).pdf $(MAIN)_lastCompile.pdf

clean:
	@rm -f $(MAIN).{pdf,ps,log,lot,lof,toc,out,dvi,blg} *.aux
	@echo Cleared all temporary files and $(MAIN).pdf

clear:
	@rm -f $(MAIN).{ps,log,lot,lof,toc,out,dvi,blg} *.aux
	@echo Cleared all temporary files

draft:
	@cp $(MAIN).pdf $(MAIN)-draft-$(DTM).pdf
	@echo Saved the draft as: $(MAIN)-draft-$(DTM).pdf

